Real-Time Constrained 6D Object-Pose Tracking of An In-Hand Suture Needle for Minimally Invasive Robotic Surgery

Autonomous suturing has been a long-sought-after goal for surgical robotics. Outside of staged environments, accurate localization of suture needles is a critical foundation for automating various suture needle manipulation tasks in the real world. When localizing a needle held by a gripper, previous work usually tracks them separately without considering their relationship. Because of the significant errors that can arise in the stereo-triangulation of objects and instruments, their reconstructions may often not be consistent. This can lead to unrealistic tool-needle grasp reconstructions that are infeasible. Instead, an obvious strategy to improve localization would be to leverage constraints that arise from contact, thereby constraining reconstructions of objects and instruments into a jointly feasible space. In this work, we consider feasible grasping constraints when tracking the 6D pose of an in-hand suture needle. We propose a reparameterization trick to define a new state space for describing a needle pose, where grasp constraints can be easily defined and satisfied. Our proposed state space and feasible grasping constraints are then incorporated into Bayesian filters for real-time needle localization. In the experiments, we show that our constrained methods outperform previous unconstrained/constrained tracking approaches and demonstrate the importance of incorporating feasible grasping constraints into automating suture needle manipulation tasks.

==> sections/draft.tex <==
\section{Draft}

\begin{equation}
\begin{aligned}
    \textrm{Track} \quad & p(\mathbf{p}_t | \mathbf{o}_{0:t}) \\
    \textrm{where} \quad & \mathbf{p}_t =\mathbf{p}_{t-1} + \mathbf{w}_t \sim \mathcal{W}(\cdot | \mathbf{p}_{t-1}) \\
    & \mathbf{o}_t \sim \mathcal{V}_t(\cdot | \mathbf{p}_t) \\
    & \mathbf{p}_t \sim \psi_t(\cdot | \mathbf{p}_{t-1}) \\
    & \ell_t = \mathcal{L}(\mathbf{p}_t) + u_t, u_t \sim \varphi(\cdot) \\
    & \left| \mathcal{L}(\mathbf{p}_t) - \mathcal{L}(\mathbf{p}^*) \right| \leq \varepsilon, \forall t \geq T \\
\end{aligned}
\end{equation}

==> sections/related_work.tex <==
\section{Related Work}

\cite{ozguner2018three}: track 6D pose with particle filter; use stereo images, robot kinematics; allow tracking under occlusion; assume the initial pose of the needle is known; needle in an image is segmented using proposed thin feature segmentation; requires virtually rendering the whole needle image
